DTR-Bench: An in silico Environment and Benchmark Platform for Reinforcement Learning Based Dynamic Treatment Regime

Reinforcement learning (RL) has garnered increasing recognition for its potential to optimise dynamic treatment regimes (DTRs) in personalised medicine, particularly for drug dosage prescriptions and medication recommendations. However, a significant challenge persists: the absence of a unified framework for simulating diverse healthcare scenarios and a comprehensive analysis to benchmark the effectiveness of RL algorithms within these contexts. To address this gap, we introduce \textit{DTR-Bench}, a benchmarking platform comprising four distinct simulation environments tailored to common DTR applications, including cancer chemotherapy, radiotherapy, glucose management in diabetes, and sepsis treatment. We evaluate various state-of-the-art RL algorithms across these settings, particularly highlighting their performance amidst real-world challenges such as pharmacokinetic/pharmacodynamic (PK/PD) variability, noise, and missing data. Our experiments reveal varying degrees of performance degradation among RL algorithms in the presence of noise and patient variability, with some algorithms failing to converge. Additionally, we observe that using temporal observation representations does not consistently lead to improved performance in DTR settings. Our findings underscore the necessity of developing robust, adaptive RL algorithms capable of effectively managing these complexities to enhance patient-specific healthcare. We have open-sourced our benchmark and code at https://github.com/GilesLuo/DTR-Bench.

==> tables/table_env_summary.tex <==
    \begin{tabular}{c|c|c|c|c}
    \hline
    Environment & Disease &  Treatment & Dynamics& Action Space \\
    \hline
      \textit{AhnChemoEnv} & Cancer & Chemotherapy & ODE& Cont./Disc. \\
      \textit{GhaffariCancerEnv} & Cancer & Chemotherapy \& Radiotherapy & ODE& Cont./Disc. \\
      \textit{OberstSepsisEnv} & Sepsis & Antibiotics, Mechanical Ventilation, Vasopressors & SCM& Disc. \\
    \textit{SimGlucoseEnv} & Type-1 Diabetes & Insulin Administration & ODE& Cont./Disc. \\
    \hline       
    \end{tabular}

==> tables/table_result.tex <==
%%%%%%%%%%%%%%%%%%%%%% OberstSepsis %%%%%%%%%%%%%%%%
\begin{longtable}{ c c| c c}
\small
\caption{Test Results on OberstSepsisEnv for 5 discrete policies and 4 RNN-based discrete policies}\\
\hline
Policy & Setting & Reward & Length\\
\hline
\endfirsthead

\multicolumn{4}{c}%
{\tablename\ \thetable\ -- \textit{Continued from previous page}} \\
\hline
Policy & Setting & Reward (mean $\pm$ std) & Length\\
\hline
\endhead

\hline
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot

\hline
\endlastfoot

\multirow{5}{*}{DQN} & 1 & $0.1515 \pm 0.7297$ & 24.0042 \\
& 2 & $0.1180 \pm 0.7382$ & 24.0365 \\
& 3 & $0.1405 \pm 0.7379$ & 23.7606 \\
& 4 & $0.0770 \pm 0.7141$ & 25.5960 \\
& 5 & $-0.0823 \pm 0.4610$ & 34.6131 \\
\hline
\multirow{5}{*}{DDQN} & 1 & $0.1692 \pm 0.7314$ & 23.7497 \\
& 2 & $0.1484 \pm 0.7336$ & 23.8056 \\
& 3 & $0.1412 \pm 0.6972$ & 25.7525 \\
& 4 & $0.0914 \pm 0.7321$ & 24.8200 \\
& 5 & $-0.1192 \pm 0.5668$ & 31.8902 \\
\hline
\multirow{5}{*}{DDQN-dueling} & 1 & $0.1575 \pm 0.7454$ & 23.2262 \\
& 2 & $0.1628 \pm 0.7235$ & 24.3151 \\
& 3 & $0.1416 \pm 0.7179$ & 24.8747 \\
& 4 & $0.0946 \pm 0.7202$ & 25.2215 \\
& 5 & $-0.0765 \pm 0.5162$ & 33.2581 \\
\hline
\multirow{5}{*}{C51} & 1 & $0.1298 \pm 0.7178$ & 24.6832 \\
& 2 & $0.0836 \pm 0.6445$ & 27.8255 \\
& 3 & $0.0233 \pm 0.4951$ & 33.0524 \\
& 4 & $0.0506 \pm 0.6546$ & 28.3496 \\
& 5 & $-0.0462 \pm 0.2672$ & 37.9895 \\
\hline
\multirow{5}{*}{discrete-SAC} & 1 & $0.1628 \pm 0.7119$ & 24.4182 \\
& 2 & $0.1579 \pm 0.7165$ & 24.2200 \\
& 3 & $0.1240 \pm 0.7106$ & 24.8654 \\
& 4 & $0.0606 \pm 0.6545$ & 28.1126 \\
& 5 & $-0.0643 \pm 0.3090$ & 37.1244 \\
\hline
\multirow{5}{*}{DQN-rnn} & 1 & $-0.1079 \pm 0.7700$ & 19.5607 \\
& 2 & $-0.2226 \pm 0.6231$ & 24.5445 \\
& 3 & $-0.1873 \pm 0.7412$ & 20.0138 \\
& 4 & $-0.1922 \pm 0.7011$ & 22.0412 \\
& 5 & $-0.2714 \pm 0.5282$ & 27.3080 \\
\hline
\multirow{5}{*}{DDQN-rnn} & 1 & & \\
& 2 & $-0.1548 \pm 0.7707$ & 18.9751 \\
& 3 & $-0.2508 \pm 0.6923$ & 21.4364 \\
& 4 & $-0.1697 \pm 0.7370$ & 20.3346 \\
& 5 & $-0.2915 \pm 0.5299$ & 26.9498 \\
\hline
\multirow{5}{*}{C51-rnn} & 1 & $-0.6756 \pm 0.5065$ & 15.9368 \\
& 2 & $-0.3508 \pm 0.4784$ & 28.4520 \\
& 3 & $-0.2500 \pm 0.4344$ & 31.2524 \\
& 4 & $-0.1559 \pm 0.3657$ & 34.6981 \\
& 5 & $-0.4257 \pm 0.5304$ & 24.2013 \\
\hline
\multirow{5}{*}{discrete-SAC-rnn} & 1 & $0.1735 \pm 0.5224$ & 29.7376 \\
& 2 & $-0.0370 \pm 0.2641$ & 37.3956 \\
& 3 & $0.1465 \pm 0.4780$ & 31.1857 \\
& 4 & $-0.0825 \pm 0.3048$ & 36.2685 \\
& 5 & $-0.1466 \pm 0.3570$ & 34.3744 \\

\end{longtable}

%%%%%%%%%%%%%%%%%%%%%% AhnChemoEnv %%%%%%%%%%%%%%%%
\newpage
\begin{longtable}{c c| c c}
\caption{Test Results on AhnChemoEnv for 5 discrete policies, 4 RNN-based discrete policies, and 3 continuous policies}\\
\hline
Policy & Setting & Reward (mean $\pm$ std) & Length\\
\hline
\endfirsthead

\multicolumn{4}{c}%
{\tablename\ \thetable\ -- \textit{Continued from previous page}} \\
\hline
Policy & Setting & Reward & Length\\
\hline
\endhead

\hline
\multicolumn{4}{r}{\textit{Continued on next page}} \\
\endfoot

\hline
\endlastfoot

\multirow{5}{*}{DQN} & 1 & $214.1753 \pm 141.6369$ & 600.0000 \\
& 2 & $129.2374 \pm 367.5353$ & 376.3382 \\
& 3 & $142.3609 \pm 366.1009$ & 381.0017 \\
& 4 & $95.7621 \pm 389.0007$ & 393.7986 \\
& 5 & $126.5550 \pm 394.2213$ & 403.1680 \\
\hline
\multirow{5}{*}{DDQN} & 1 & $370.6112 \pm 18.3647$ & 600.0000 \\
& 2 & $170.0178 \pm 375.1586$ & 438.2222 \\
& 3 & $132.9528 \pm 381.9179$ & 403.8939 \\
& 4 & $134.3563 \pm 376.1076$ & 385.5776 \\
& 5 & $131.9622 \pm 389.6840$ & 401.1204 \\
\hline
\multirow{5}{*}{DDQN-dueling} & 1 & $248.5918 \pm 66.7666$ & 600.0000 \\
& 2 & $95.0447 \pm 349.6679$ & 341.3426 \\
& 3 & $97.4903 \pm 363.6415$ & 336.5172 \\
& 4 & $105.2156 \pm 344.0574$ & 316.8232 \\
& 5 & $87.4417 \pm 354.0185$ & 321.4076 \\
\hline
\multirow{5}{*}{C51} & 1 & $144.2966 \pm 90.1000$ & 600.0000 \\
& 2 & $108.0523 \pm 344.9694$ & 357.9451 \\
& 3 & $141.8950 \pm 356.6314$ & 378.5530 \\
& 4 & $122.5256 \pm 377.3599$ & 383.7680 \\
& 5 & $128.0521 \pm 386.8756$ & 398.2884 \\
\hline
\multirow{5}{*}{discrete-SAC} & 1 & $114.0624 \pm 82.6777$ & 600.0000 \\
& 2 & $137.8815 \pm 404.3628$ & 448.8814 \\
& 3 & $112.6139 \pm 372.1017$ & 380.2625 \\
& 4 & $124.1409 \pm 385.2034$ & 392.3511 \\
& 5 & $132.3392 \pm 357.6143$ & 371.2976 \\
\hline
\multirow{5}{*}{DQN-rnn} & 1 & $267.7758 \pm 62.6521$ & 600.0000 \\
& 2 & $113.8996 \pm 352.3412$ & 356.3033 \\
& 3 & $115.4531 \pm 355.8717$ & 370.5290 \\
& 4 & & \\
& 5 & $91.1298 \pm 368.6296$ & 367.4828 \\
\hline
\multirow{5}{*}{DDQN-rnn} & 1 & $317.3427 \pm 35.2439$ & 600.0000 \\
& 2 & $132.6046 \pm 350.0453$ & 384.9308 \\
& 3 & $108.6286 \pm 355.7591$ & 350.6842 \\
& 4 & $101.1061 \pm 372.5984$ & 351.2267 \\
& 5 & $88.9151 \pm 342.9476$ & 301.7248 \\
\hline
\multirow{5}{*}{C51-rnn} & 1 & $242.1839 \pm 82.2905$ & 600.0000 \\
& 2 & & \\
& 3 & $38.6649 \pm 300.8929$ & 350.1939 \\
& 4 & $64.1744 \pm 331.9245$ & 373.4832 \\
& 5 & $73.4879 \pm 321.9673$ & 311.7191 \\
\hline
\multirow{5}{*}{discrete-SAC-rnn} & 1 & $341.0149 \pm 24.6316$ & 600.0000 \\
& 2 & $126.5335 \pm 378.3509$ & 457.7371 \\
& 3 & & \\
& 4 & $99.4602 \pm 391.7221$ & 417.0609 \\
& 5 & $102.3028 \pm 389.9677$ & 418.6284 \\
\hline
\multirow{5}{*}{DDPG} & 1 & $113.2838 \pm 55.9263$ & 600.0000 \\
& 2 & $80.9527 \pm 327.3295$ & 297.7201 \\
& 3 & $80.7243 \pm 342.7315$ & 310.6698 \\
& 4 & $124.6685 \pm 376.7492$ & 419.2463 \\
& 5 & $102.4956 \pm 349.7174$ & 345.0929 \\
\hline
TD3 & 1 & $90.3175 \pm 54.0430$ & 600.0000 \\
\multirow{4}{*}{TD3}& 2 & $82.1043 \pm 339.2868$ & 314.9694 \\
& 3 & $92.6817 \pm 357.9982$ & 345.9679 \\
& 4 & $87.3757 \pm 344.4031$ & 350.4695 \\
& 5 & $76.9739 \pm 347.4834$ & 316.2588 \\
\hline
\multirow{5}{*}{SAC} & 1 & $151.7157 \pm 88.3466$ & 600.0000 \\
& 2 & $89.0880 \pm 338.3210$ & 338.2896 \\
& 3 & $99.5888 \pm 340.7931$ & 334.0368 \\
& 4 & $115.9857 \pm 363.4531$ & 370.4038 \\
& 5 & $108.8021 \pm 374.3522$ & 381.6586 \\
\hline
\end{longtable}

==> text/biography.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/zhiyao.jpg}}]{Zhiyao Luo} received his MSc. degree from National University of Singapore, and he is now working towards a DPhil Degree with the Department of Engineering Science, University of Oxford. His research interests include reinforcement learning based dynamic treatment regimes, medical sequential decision making and broader applications which bridge the gap between machine learning and clinical science. 
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/mingcheng.jpg}}]{Mingcheng Zhu} received his MRes degree from Imperial College London and will be pursuing a DPhil at the Department of Engineering Science, University of Oxford. His research interests lay in domain adaptation for AI-Healthcare, particularly concerning time-series clinical records.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{photos/fenglin.jpg}}]{Fenglin Liu} 
is a PhD student at the University of Oxford, where he is supervised by Professor David A. Clifton.
His research interests include Natural Language Processing, Machine Learning, and their applications to healthcare. He has published papers at premier journals and conferences and served on many review committees for top-tier venues, e.g., Nature Medicine, TPAMI, NeurIPS, ICML, ICLR, ACL, EMNLP, NAACL, CVPR, ICCV, and ECCV.
He was awarded as the Distinguished Reviewer of CVPR, ACL, AAAI, and IJCAI.
\end{IEEEbiography}

